Data-Uncertainty Guided Multi-Phase Learning for Semi-Supervised Object Detection

In this paper, we delve into semi-supervised object detection where unlabeled images are leveraged to break through the upper bound of fully-supervised object detection models. Previous semi-supervised methods based on pseudo labels are severely degenerated by noise and prone to overfit to noisy labels, thus are deficient in learning different unlabeled knowledge well. To address this issue, we propose a data-uncertainty guided multi-phase learning method for semi-supervised object detection. We comprehensively consider divergent types of unlabeled images according to their difficulty levels, utilize them in different phases and ensemble models from different phases together to generate ultimate results. Image uncertainty guided easy data selection and region uncertainty guided RoI Re-weighting are involved in multi-phase learning and enable the detector to concentrate on more certain knowledge. Through extensive experiments on PASCAL VOC and MS COCO, we demonstrate that our method behaves extraordinarily compared to baseline approaches and outperforms them by a large margin, more than 3% on VOC and 2% on COCO.

==> zhushi <==
%It has been observed that deep neural networks are prone to fit any labels, even completely noisy ones \cite{zhang2016understanding}. We find that detection models are also easy to fit noise within pseudo labels. We use VOC 2007 trainval as labeled set and VOC 2012 trainval as unlabeled set to execute self-training SSOD twice. Different models from different phases are evaluated on training data and testing data separately. The results are in Fig. \ref{fig:ofd}.




%Because of this problem, the performance is hard to improve if SSOD continues with more phases. If we apply the SSOD model from the first phase to generate new pseudo labels and conduct SSOD in the second time, as in Fig. \ref{fig:21}, the quality of new pseudo labels drops, a consequence of lower mAP on VOC12 trainval, causing test mAP decline in the second phase. We conclude that during SSOD training, the generalization ability of the model is strengthened while its detection ability on unlabeled training dataset is weakened. Therefore, traditional pseudo labels based semi-supervised methods are hard to be performed in multiple phases without performance reduction.


%We select some images to further explain this problem. The examples are in Fig. \ref{fig:of}. In the first case, the supervised model mislabels the aeroplane as a car, and we notice that the semi-supervised model trained with this pseudo label detects one more car that does not exist. In the second case, the supervised model thinks a part of iron mesh is a person. This may be an accident mistake. However, in the results from semi-supervised model, more parts of iron mesh are detected as persons. Actually, noise within pseudo labels offers as wrong supervised information to guide new model during training. New model will take this wrong knowledge as correct one and try to mimic it, so noise in pseudo labels is amplified. This is the fundamental reason why previous SSOD method can only be performed once.

%Overlap Based Soft-Sampling mitigates missing annotation problem to some extent. However, this method can hardly be applied to SSOD. The main reason is the choice of $a$. According to Eq. \ref{eqa:ss}, $a$ is approximately the value when IoU is close to 0 since $b$ is usually a large number. $a$ is set to 0.25 in practice, so a small part of incorrect gradients can still back-propagate and affect the network. But if $a$ is set with a smaller value, some correct information will be reduced too. As a result, 0.25 is a compromising value for $a$. This causes that incorrect gradients are not reduced enough in Overlap Based Soft-sampling method.

%Actually, Overlap Based Soft-sampling aims to reduce gradients of uncertain RoIs. It treats IoUs with other positive instances as a metric of uncertainty, which is too naive for SSOD. 


It selects images that detectors are more certain about and enables that detection models are certain about each annotation in pseudo labels. Images with a small $\overline{s_m}$ are regarded as difficult images and are filtered for training in the first several phases. Then detectors will not be distracted by uncertain images and can center on more certain \emph{images} to mitigate label noise overfitting problem.

%Above scheme, however, can only conduct self-training learning once and cannot proceed continuously. The reason lies in noise within pseudo labels. Deep learning based model is easy to fit any training annotation, even the wrong one. When pseudo labels contain some false information, detection model is also able to "learn" it. We call this phenomenon label noise overfitting problem. If we execute SSOD twice or more directly, the quality of pseudo labels declines, leading to performance reduction of models trained in later steps. This will be explained detailedly in section \ref{nl}.

%These models can be naturally generated from different training phases. Therefore, a multi-phase SSOD learning approach is urgently needed to settle above issues.

%This is useful to some extent because this kind of images is often difficult and contain information that detection model has not ever learned before. But label noise overfitting problem also makes the model easier to overlook other simple images which are also helpful. In a word, one semi-supervised learning step model can only describe difficult data with more noise accurately and cannot fit easy unlabeled images equally well. Because of above reasons, it is challenging to use a single model embedding simple and difficult feature meanwhile. A simplest solution is to use multiple models encoding simple or difficult information respectively, and ensemble them together. These models can be naturally generated from different training steps. Therefore, a multi-step SSOD learning method is urgently needed to settle above issues.

%Label noise overfitting problem is an essential feature of deep learning model thus hardly to be solved. Therefore, a multi-step SSOD learning method is urgently needed to settle above problems

It has been previously observed \cite{arpit2017closer, zhang2016understanding, ma2018dimensionality} that deep learning based models are susceptible to memorize any training annotations, even noisy ones. 

We believe this problem is hard to be well solved with just one SSOD model. Even if we adopt some techniques to force the model to concentrate on easy images, difficult uncertain images cannot be described accurately at the same time, an effect of deep learning model's different fitting ability to certain and uncertain information. 


%\begin{table*}[]
%\centering
%\setlength{\abovecaptionskip}{0pt}
%\setlength{\belowcaptionskip}{0pt}
%\caption{ \textbf{Illustration of label noise overfitting problem for detection models.} Supervised model is trained on VOC07 trainval. Semi-supervised model 1 uses pseudo labels from supervised model, and semi-supervised model 2's pseudo labels are from semi-supervised model 1.}
%\resizebox{1.8\columnwidth}{!}{
%\begin{tabular}{c|c|c|c|c|c|c}
%\Xhline{1.2pt}
%Model &  \tabincell{c}{VOC07\\Test} & \tabincell{c}{VOC12\\Trainval} & \tabincell{c}{VOC07 \\ Trainval} & \tabincell{c}{VOC12 Trainval \\ Pseudo Labels} & \tabincell{c}{VOC07 Test \\ (easy)} & \tabincell{c}{VOC07 Test \\ (difficult)}\\
%\hline
%Supervised Model  & 74.8   & 69.0 & 90.5 & - & 86.2 & 59.1\\
%Semi-Supervised Model 1  &  75.6  & 66.6 & 90.2 & 97.4 & 85.8 & 61.1\\
%Semi-Supervised Model 2  &  75.1  & 66.2 & 89.6 & 98.4 & 85.7 & 60.9 \\
%\Xhline{1.2pt} 
%\end{tabular}
%}
%\label{tab:overfitting}
%\end{table*}


%\begin{figure}[]
%   \centering
%   \setlength{\abovecaptionskip}{0pt}
%   \setlength{\belowcaptionskip}{0pt}
%   \includegraphics[width=\columnwidth]{images/of.jpg}
%   \caption{\textbf{Examples to explain label noise overfitting problem.} The left column is pseudo labels from supervised model, and the right column is from semi-supervised model trained with pseudo labels from supervised model.}
%   \label{fig:of}
%   \setlength{\abovecaptionskip}{0pt}
%   \setlength{\belowcaptionskip}{0pt}
%\end{figure}




%The overall process can be seen in Algorithm \ref{alg:process}, where we use a two-step process to explain our method. The above process can of course extend to more processes. We will illustrate it in experiments part.

%After training, we obtain a series of models. They are expert in different levels of difficult knowledge. Concretely, model B in Algorithm \ref{alg:process} learns simple information better. So during inference, if the image is relatively straightforward, model B is more suitable for tackling it. While model trained with all data (model C) is easy to fit to difficult information so is more suitable for difficult images from test set. Therefore, it is better to use all models for inference. We use weighted boxes fusion method \cite{solovyev2019weighted} to ensemble detection results from all models (model A, B and C). In this way, different types of information can be utilized synthetically thus the overall performance is improved.


%From above analysis, the reason why previous semi-supervised object detection method using pseudo labels cannot be performed in multiple steps is the noisy labels overfitting problem. This problem is because the noise from pseudo labels. However, the noise in pseudo labels cannot be removed. If we correct the mistakes in pseudo labels, we can also perform this process in training fully-supervised model to improve its performance. Considering fully-supervised object detection has been researched extensively but it still cannot achieve a result close to 100\%, we think that the errors in pseudo labels is hard to correct.

%Although the noise cannot be eliminated, we can try to avoid it. In a particular dataset, there exists both simple images and difficult images. For simple images, the pseudo labels on them will have less noise and are more likely to be correct, while for difficult images, the pseudo labels will be more noisy. If we can pick simple images out, the pseudo labels will be relatively clean, then the noisy labels overfitting problem may be avoided.

%Therefore, we need a method to estimate the difficulty level for an image. For a simple image, the detection model should be sure of any objects inside it. Using $\left\{ (bb_{ij}, p_{ij}) \right\}_{j=1}^M$ to denote the bounding boxes (i.e. pseudo labels) in Image $I_i$, where $bb_{ij}$ is the bounding box and $p_{ij}$ is the corresponding score, of course $p_{ij}$ can represents how certain the detection model is about the bounding box, that is, the difficulty degree. So we use the average of scores of all bounding boxes inside an image to measure its difficulty:


%\subsection{Results Ensembling}

%Using $m_i$ from Eq. \ref{equ:diff}, we can pick simple images from an unlabeled dataset. Then, we can use labeled images and pseudo labels on simple images to perform semi-supervised object detection first. This model is less likely to be affected by noisy labels overfitting problem. Then, this model can be used for subsequent training. Of course, the pseudo labels from this model trained with labeled data and simple unlabeled data can be directly used for later use. However, since we have not only this semi-supervised detection model but also the initial supervised detection model, it is better to consider results from both models.


%Considering that we have proposed our UWL to improve missing annotations problem, the model should be more sensitive to false annotations, rather than missing annotations. So when ensembling pseudo labels from multiple models for later training, we should try to improve the precision of pseudo labels, rather than the recall. Taking \emph{intersection} of several pseudo labels is a simple and effective way. As a result, for a particular bounding box, we will only use it if it appears in pseudo labels from all models. In this way, we can perform semi-supervised object detection in multiple iterations. The overall process can be seen in Algorithm \ref{alg:process}, where we use a two-step process to explain our method. The above process can of course extend to more processes. We will illustrate it in experiments part.

%After training, the ultimate semi-supervised detection model has an excellent ability and can be applied for testing. However, these models are trained on different data so their information is complementary to each other, especially for model trained with just simple images (model B in Algorithm \ref{alg:process}) and model trained with all data (model C). In inference time, if the image is relatively straightforward, model B is more suitable for tackling it, and vice versa. Therefore, it is better to use all models for inference. We use weighted boxes fusion method \cite{solovyev2019weighted} to ensemble detection results from all models (model A, B and C). In this way, different types of information can be utilized synthetically thus the overall performance is improved. %Since detection models for different steps are the same, the backbone parameters in model A, B, and C are closely similar to each other. So we can actually use the same backbone. As a result, the inference speed actually would not be reduced significantly.

%\begin{table}[]
%\centering
%\setlength{\abovecaptionskip}{0pt}
%\setlength{\belowcaptionskip}{0pt}
%\caption{\textbf{Multiple phases semi-supervised learning on VOC07 test.} Learning process is the performance of models obtained from each phases, and ensembled mAP is the ultimate ensembled result. }
%\resizebox{\columnwidth}{!}{
%\begin{tabular}{c|c|c}
%\Xhline{1.2pt}
%Steps & Learning Process & Ensembled mAP \\
%\hline
%2 &  76.6 $\rightarrow$ 77.4 & 78.6 \\
%3 &  75.9 $\rightarrow$ 76.8 $\rightarrow$ 77.4   & 78.9\\
%4 &  75.8 $\rightarrow$ 76.6 $\rightarrow$ 76.9 $\rightarrow$ 77.2  & 78.9 \\

%\Xhline{1.2pt} 
%\end{tabular}
%}
%\label{tab:morestep}
%\end{table}

%But IoU is not enough for describing uncertainty of RoIs. When objects are relatively sparse, almost all negative RoIs have a close-to-zero IoU with positive regions. When objects are close to each other and almost fill the whole image, IoUs are always large. In these quite common situations, almost all negative regions are treated equally. They have the same uncertainty degree, which is of no sense. Apparently, similarity between different RoIs is a necessary metric for uncertainty - if a region has a high similarity with an existing object but has no groundtruth labels, we can assert that it is more uncertain. We use cosine distance to calculate similarity between different RoIs. Let $f_i$ denote the feature of RoI$_i$. The distance (\emph{i.e.} dissimilarity) $d_{ij}$ between RoI$_i$ and RoI$_j$ is:

%For RoI$_i$, above $D_i$ is small when it is similar to a positive RoI which does not cover RoI$_i$. This is a good description for similarity based uncertainty.


%\begin{figure}[]
%   \centering
%   \setlength{\abovecaptionskip}{0pt}
%   \setlength{\belowcaptionskip}{0pt}
%   \includegraphics[width=\columnwidth]{images/diff.jpg}
%   \caption{\textbf{Examples to explain difference between different models.} The left column is results from the first phase model and the second column is from the second phase model.}
%   \label{fig:diff}
%   \setlength{\abovecaptionskip}{0pt}
%   \setlength{\belowcaptionskip}{0pt}
%\end{figure}
